Symbol Resolution MatRs: Make it Fast and Observable with Stable Linking

Dynamic linking is the standard mechanism for using external dependencies since it enables code reuse, streamlines software updates, and reduces disk/network use. Dynamic linking waits until runtime to calculate an application's relocation mapping, i.e., the mapping between each externally referenced symbol in the application to the dependency that provides the symbol. Unfortunately, it comes with two downsides. First, dynamic linking limits the performance of current systems since it can take seconds to calculate a relocation mapping for a large program. Second, dynamic linking limits the dependency management of applications since it prevents a developer from accurately observing a relocation mapping except at runtime. This paper makes the key insight that the benefits conventionally attributed to dynamic linking: code reuse, streamlined software updates, and reduced disk/network use are actually benefits of shared libraries. Thus, we present stable linking, a new mechanism for using dependencies that uses shared libraries to retain their benefits but eliminates the downsides of dynamic linking. Stable linking separates a system's state into management times; when the system can be modified, and epochs when it cannot. Stable linking calculates each application's relocation mapping at the beginning of each epoch, allows developers to inspect the relocation mapping during the epoch, and reuses the mapping for subsequent executions in the epoch. We design and build MatR, the first stable linker. We use MatR in three workloads and show that it improves upon dynamic linking performance by a factor of 2.19 on average. Additionally, we use the system in three vignettes, or case-studies, that illustrate the system's improvements to dependency management.

==> intro-outline.tex <==
1. Dynamic linking is the de-facto way in which software is built
  * What is dynamic linking?
  * Examples of why we use dependencies/dynamic linking
  * The number of dependencies is growing and/or code is more complex
  * Make sure to define each external library using the word "dependency".
  * Why we like dynamic linking...

2. Alas, dynamic linking limits the performance and dependency management functionality of today's applications.
  * Focusing on performance,...
  * Elaborate prior work on dynamic linking performance optimizations.

3. Focusing on Dependency management.
  * Visibility point---what am I linking? 
  * Granularity point---can I update/change a single function?
  * Update point---what am I updating? (compatability)
  * Elaborate on prior work and its limitations.

3. In this paper, we introduce a new property for dependency tracking called stability as an enabler for solving the performance and dependency management challenges imposed by dynamic linking.
  * A dependency tracking system is stable if the system only updates dependencies at well-defined times, called management times. 
  * Explain why this is helpful.
  * Explain how current package managers provide the features required to facilitate stability already.
  * We introduce a new principle/property, stable dependency systems, for which the system is stable (unchanged) across
  * Most systems use package managers that already provide the features needed for stability
  * Well defined times when dependencies are updated---introduce the term "management time".
  facilitate
  * Loader is stable.
  * Reference human behavior in some way as facilitating stability.

4. Then, we present a new dependency management system that exploits stability, called \sys{} (\underline{Mate}rialized \underline{R}elocations), that improves the performance and dependency management of the dynamic linking process. 
  * High level idea of what Mater does. 
  (avoid using word cache)
    
5. We built a prototype of \sys{} by extending musl and using Nix to provide stability. 
   * Paragraph previews performance results.
   * Include actual numbers and some notion of the experiments that we ran.

6. Paragraph previewing management results
  * Include details of each of the vignettes that we perform.
  * Include any examples we can find of updates gone wrong (e.g., any blogs or something about a bad update taking down a system that would be caught by MATER).

7. Paragraph pointing at larger impact of no longer needing lazy loading.
  * Include performance results for dropping the PLT.
  * Point to potential to drop GOT from our systems and cite the potential for improved security (in certain cases).

In summary, our contributions are: 
\begin{enumerate}
\item The stability property for dependency systems, which enables improved dependency performance and management by exploiting usage patterns employed by many of today's system administrators. 
\item The design and implement of \sys{}, which exploits stability to improve dependency performance and management.
\item An evaluation of \sys{} showing that it improves dependency performance and management.
\end{enumerate}
  

==> text/management_time_diagram.tex <==
\begin{sequencediagram}
    \newthread{sys}{System}
    \newinst{mater}{\sys{}}
    \newinst{lib}{:Library}
    \newinst{exec}{:Executable}
    \begin{sdblock}[green!20]{ Management Time }{ }
        \mess[0]{sys}{begin}{mater}
        \begin{messcall}{sys}{update}{mater}
            \mess[0]{mater}{record}{lib}
        \end{messcall}
        \begin{messcall}{sys}{update}{mater}
            \mess[0]{mater}{record}{exec}
        \end{messcall}
        \begin{messcall}{sys}{end}{mater}
            \begin{call}{mater}{calculate()}{mater}{}
            \end{call}
        \end{messcall}
    \end{sdblock}
    \mess{sys}{exec}{exec}
\end{sequencediagram}
